Efficiency of Magnetic to Kinetic Energy Conversion in a Monopole Magnetosphere

Unconfined relativistic outflows from rotating, magnetized compact objects are often well-modeled by assuming the field geometry is approximately a split-monopole at large radii. Earlier work has indicated that such an unconfined flow has an inefficient conversion of magnetic energy to kinetic energy. This has led to the conclusion that ideal magnetohydrodynamical (MHD) processes fail to explain observations of, e.g., the Crab pulsar wind at large radii where energy conversion appears efficient. In addition, as a model for astrophysical jets, the monopole field geometry has been abandoned in favor of externally confined jets since the latter appeared to be generically more efficient jet accelerators. We perform time-dependent axisymmetric relativistic MHD simulations in order to find steady state solutions for a wind from a compact object endowed with a monopole field geometry. Our simulations follow the outflow for 10 orders of magnitude in distance from the compact object, which is large enough to study both the initial "acceleration zone" of the magnetized wind as well as the asymptotic "coasting zone." We obtain the surprising result that acceleration is actually {\it efficient} in the polar region, which develops a jet despite not being confined by an external medium. Our models contain jets that have sufficient energy to account for moderately energetic long and short gamma-ray burst (GRB) events (~10^{51}--10^{52} erg), collimate into narrow opening angles (opening half-angle \theta_j \approx 0.03 rad), become matter-dominated at large radii (electromagnetic energy flux per unit matter energy flux \sigma<1), and move at ultrarelativistic Lorentz factors (\gamma_j ~ 200 for our fiducial model). (abridged)

==> macros.tex <==
\newcommand\aj{\rmfamily{AJ}}%
          % Astronomical Journal
\newcommand\araa{\rmfamily{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\rmfamily{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\rmfamily{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\rmfamily{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\rmfamily{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\rmfamily{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\rmfamily{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\rmfamily{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\rmfamily{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\rmfamily{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\rmfamily{BAAS}}%
          % Bulletin of the AAS
\newcommand\jrasc{\rmfamily{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\rmfamily{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\rmfamily{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\pra{\rmfamily{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\rmfamily{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\rmfamily{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\rmfamily{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\rmfamily{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\rmfamily{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasp{\rmfamily{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\rmfamily{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\rmfamily{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\skytel{\rmfamily{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\rmfamily{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\rmfamily{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\rmfamily{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\rmfamily{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\rmfamily{Nature}}%
          % Nature
\newcommand\iaucirc{\rmfamily{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\rmfamily{Astrophys.~Lett.}}%
          % Astrophysics Letters
\newcommand\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\rmfamily{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\rmfamily{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\rmfamily{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\rmfamily{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\rmfamily{J.~Geophys.~Res.}}%
          % Journal of Geophysics Research
\newcommand\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\rmfamily{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\rmfamily{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\rmfamily{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\rmfamily{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\rmfamily{Proc.~SPIE}}%
          % Proceedings of the SPIE
